The challenges of temporal alignment on Twitter during crises

Language use changes over time, and this impacts the effectiveness of NLP systems. This phenomenon is even more prevalent in social media data during crisis events where meaning and frequency of word usage may change over the course of days. Contextual language models fail to adapt temporally, emphasizing the need for temporal adaptation in models which need to be deployed over an extended period of time. While existing approaches consider data spanning large periods of time (from years to decades), shorter time spans are critical for crisis data. We quantify temporal degradation for this scenario and propose methods to cope with performance loss by leveraging techniques from domain adaptation. To the best of our knowledge, this is the first effort to explore effects of rapid language change driven by adversarial adaptations, particularly during natural and human-induced disasters. Through extensive experimentation on diverse crisis datasets, we analyze under what conditions our approaches outperform strong baselines while highlighting the current limitations of temporal adaptation methods in scenarios where access to unlabeled data is scarce.

==> sections/ethics.tex <==
\section*{Ethics Statement}

==> sections/tab_all.tex <==
% Results Table goes here.

\begin{table*}[h!]
	\small
	\begin{center}
		\begin{tabular}{l S S S S S S S S S}
			\toprule
			
			\multirow{2}{*}{Method} & \multicolumn{3}{c}{\sandy} & \multicolumn{3}{c}{\clex} & \multicolumn{3}{c}{\humaid} \\ 
			
			\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
			
			& \textsc{cont} & \textsc{temp} & \textsc{diff} & \textsc{cont} & \textsc{temp} & \textsc{diff} & \textsc{cont} & \textsc{temp} & \textsc{diff} \\
			
			\toprule
			%\toprule
			%\hline
			BASE & 0.8689 & 0.8057 & 0.0632 & 0.4124 & 0.3708 & 0.0416 & 0.403 & 0.3616 & 0.0414 \\
			
			%\toprule
			\midrule
			
            DCWE & 0.8659 & 0.7857 & 0.0802 & 0.3533 & 0.3184 & 0.0349 & 0.323 & 0.2889 & 0.0341 \\
			
			
			TAPH & 0.8677 & 0.8135 & 0.0542 & 0.3424 & 0.3187 & 0.0237 & 0.3209	& 0.2827 & 0.0382 \\
			
			
			TDA & 0.8615 & 0.8147 & 0.0468 & 0.3949 & 0.3491 & 0.0458 & 0.3883 & 0.3214 & 0.0669\\
			
			\midrule
			
			MLM + BASE & 0.8634 & 0.8156 & 0.0478 & 0.4204 & 0.3902 & 0.0301 & 0.4408 & 0.4193 & 0.0214 \\
			
			\midrule
			
			MLM + DCWE & 0.8748 & 0.8030 & 0.0717 & 0.3838 & 0.3426 & 0.0412 & 0.3788 & 0.3304 & 0.0484 \\
			
			MLM + TAPH & 0.8637 & 0.8087 & 0.0549 & 0.3823 & 0.3426 &	0.0397 & 0.3910	& 0.3472 & 0.0437 \\
			
			MLM + TDA & 0.8571 & 0.8277 & 0.0294 & 0.7480 & 0.7070 & 0.0409 & 0.6902 & 0.6266 & 0.0636\\
			
			\midrule
			
			DATED & 0.8138 & 0.6938 & 0.12 & 0.4179 & 0.3887 & 0.0292 & 0.4383 & 0.41 & 0.0283 \\
			
			
			\bottomrule
			
		\end{tabular}
		\caption{\label{tab:all-res} F1 performance metric of the proposed temporal adaptation models (section \ref{sec:models}) in \textsc{control(cont)} and \textsc{temporal(temp)} setting for \sandy, \clex and \humaid datasets. For each model, we additionally report the performance difference (\textsc{diff}) between \textsc{cont} and \textsc{temp} settings. Best value in each column is highlighted in \textcolor{red}{red}. For detailed analysis refer to section \ref{sec:result}.}
	\end{center}
\end{table*}




==> src/old_results.tex <==



% Results Table goes here.
%\input{sections/tab_all}




\begin{comment}

\begin{table*}[h!]
	%\small
	\begin{center}
		\begin{tabular}{l S S S S S S S S S}
			\toprule
			
			\multirow{2}{*}{Method} & \multicolumn{3}{c}{\sandy} & \multicolumn{3}{c}{\clex{}} & \multicolumn{3}{c}{\humaid{}} \\ 
			
			\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
			
			& \textsc{cont} & \textsc{temp} & \textsc{diff} & \textsc{cont} & \textsc{temp} & \textsc{diff} & \textsc{cont} & \textsc{temp} & \textsc{diff} \\
			
			\toprule
			%\toprule
			%\hline
			BASE & \color{red}0.8689 & 0.8057 & 0.0632 & 0.4124 & 0.3708 & 0.0416 & 0.403 & 0.3616 & 0.0414 \\
			
			DCWE & 0.8659 & 0.7857 & 0.0802 & 0.3533 & 0.3184 & 0.0349 & 0.323 & 0.2889 & 0.0341 \\
			
			TAPH & 0.8677 & 0.8135 & 0.0542 & 0.3424 & 0.3187 &	\color{red}0.0237 & 0.3209	& 0.2827 & 0.0382 \\
			
			TDA & 0.8615 & \color{red}0.8147 & \color{red}0.0468 & 0.3949 & 0.3491 & 0.0458 & 0.3883 & 0.3214 & 0.0669\\
			
			BASIC	& 0.8648 & 0.8097 & 0.0551 & \color{red}0.4253 & \color{red}0.3956 & 0.0297 & 0.4365 & \color{red}0.4148 & \color{red}0.0217 \\
			
			PREPEND & 0.8138 & 0.6938 & 0.12 & 0.4179 & 0.3887 & 0.0292 & \color{red}0.4383 & 0.41 & 0.0283 \\
			
			\bottomrule
			
		\end{tabular}
		\caption{\label{tab:all-res} F1 performance metric of the proposed temporal adaptation models (section \ref{sec:models}) in \textsc{control(cont)} and \textsc{temporal(temp)} setting for \sandy{}, \clex and \humaid datasets. For each model, we additionally report the performance difference (\textsc{diff}) between \textsc{cont} and \textsc{temp} settings. Best value in each column is highlighted in \textcolor{red}{red}. For detailed analysis refer to section \ref{sec:result}.}
	\end{center}
\end{table*}

\end{comment}

%The results of the main comparison are shown in table \ref{tab:all-res}. Overall, results show that temporal adaptation models perform well when language changes rapidly in a very short time span and limited training data is available. 
%\todo{further result summary}

\begin{comment}


\subsection{Temporal Degradation} \label{subsec:temporal_degradation}

\begin{figure}[t]
	\includegraphics[width=.5\textwidth]{../assets/temporal_degradation.png}
	\centering
	\vspace{-3ex}
	\caption{\label{fig:temporal_degradation_baseline} Performance comparison between \cont and \temp setting for fine-tuned BERT baseline model. Model performance deteriorates in \temp setting due to rapid change in language in a very short time-span. For details refer to section \ref{subsec:temporal_degradation}.}
\end{figure}

To show the impact of temporal drift in language, we first compare the standard BERT baseline (see section \ref{sec:models}) model under \cont and \temp settings. We fine-tune pre-trained \texttt{bert-base-cased} embeddings using our data splits (see section \ref{sec:exp_setup}) and report the results using bar chart in figure \ref{fig:temporal_degradation_baseline}. For \clex and \humaid datasets we report mean performance score over all its constituent crisis events. 

From results in figure \ref{fig:temporal_degradation_baseline} we observe that, for every dataset the baseline model performs worse in the temporal setting. This performance drop could potentially incur extensive loss in downstream tasks with crisis data - a negative result that motivates our further study. The plausible reason behind this performance drop is the rapid language change over a very short period of time.

We also observe that model performance varies greatly between the \sandy dataset and the other two datasets. Analyzing this further, we found that unlike \clex and \humaid, \sandy dataset is larger and contains more diverse data as it is not restricted to keyword-based tweets. 

\subsection{Temporal Adaptation} \label{subsec:temporal_adaptation}

To decrease this gap between model performances in \cont and \temp settings we proposed temporal adaptation models in section \ref{sec:models}. 

In table \ref{tab:all-res} we report model performance in terms of F1 score for \cont and \temp settings across all the datasets. Additionally, for each model we report the performance difference between the \cont and \temp settings. This difference score indicates the robustness of a model towards rapid temporal drift in the languages. A score closer to zero means that the performance is similar under both \cont and \temp settings, while a higher score indicates that the model performs better under \cont setup. Nevertheless, this difference score does not give information about how suitable the proposed methods are with respect to the downstream task. In order to compare model performances with respect to a fixed reference, in figure \ref{fig:bert-base-cased-diff} we compare each model under \temp setting to the \texttt{bert-base-cased} baseline under \cont setting and report their performance difference. 

\begin{figure}[t]
	\includegraphics[width=.5\textwidth]{../assets/bert-base-cased-diff.png}
	\centering
	\vspace{-3ex}
	\caption{\label{fig:bert-base-cased-diff} Performance difference between  \texttt{bert-base-cased} in \cont setting and all the models under \temp setting. Lower score indicates performances are similar Refer to section \ref{subsec:temporal_adaptation} for detailed analysis.}
\end{figure}

Overall, the DCWE and TAPH models perform similarly to the baseline, with some improvements. However, TDA performs poorly on \clex and \humaid datasets. A plausible explanation for this is that the time span of these dataset are so short that the classification layer used for Gradient Reversal in TDA method fails to learn any useful pattern from it. 

Of all the models PREPEND variant of ALM performs worst on \sandy dataset. PREPEND processes temporal information as strings. The language changes so rapidly in that dataset that the model fails to learn patterns from the timestamps. On the contrary, for \clex and \humaid datasets domain of the data plays an important role. Hence, both BASIC and PREPEND variants of ALM performs well on these datasets. However, other models outperform ALM on these two datasets when appropriately adapted to the data domain.

\begin{figure}[t]
	\includegraphics[width=.5\textwidth]{../assets/base_temporal_bin_heatmaps.png}
	\vspace{-3ex}
	\caption{\label{fig:temp_bin_heat} Performance of BASE model on \sandy data. We train the model in \prog setting using one bin and evaluate on each of the other bins. In this case higher score is better. The heatmap is shaded per row. The darkest shade in a cell means that cell has the highest score in that row.}
	\centering
\end{figure}

In \prog setting we train each model using one bin and test on each other nine bins. We observe that the performance pattern for all the models are close. Hence, we report the performance of BASE model on \sandy dataset using heatmaps in figure \ref{fig:temp_bin_heat}. However, performance metrics vary across models, which we discuss in the following section. For performance details of the other models please refer to Appendix \ref{sec:appendixa}. 
\newline

\end{comment}
%\subsection{Continual Learning} \label{subsec:cont_learn}


%It is interesting to observe that, language modeling (BASIC variant of ALM) takes the most advantage of continual learning paradigm by gradually adapting to the language change. The available data is limited, which implies that the amount of temporal information associated to the datasets is also limited. This is the reason why the other models, which additionally process temporal information, falls behind in \prog setting.
